VideoGEM: Training-free Action Grounding in Videos

Vision-language foundation models have shown impressive capabilities across various zero-shot tasks, including training-free localization and grounding, primarily focusing on localizing objects in images. However, leveraging those capabilities to localize actions and events in videos is challenging, as actions have less physical outline and are usually described by higher-level concepts. In this work, we propose VideoGEM, the first training-free spatial action grounding method based on pretrained image- and video-language backbones. Namely, we adapt the self-self attention formulation of GEM to spatial activity grounding. We observe that high-level semantic concepts, such as actions, usually emerge in the higher layers of the image- and video-language models. We, therefore, propose a layer weighting in the self-attention path to prioritize higher layers. Additionally, we introduce a dynamic weighting method to automatically tune layer weights to capture each layer`s relevance to a specific prompt. Finally, we introduce a prompt decomposition, processing action, verb, and object prompts separately, resulting in a better spatial localization of actions. We evaluate the proposed approach on three image- and video-language backbones, CLIP, OpenCLIP, and ViCLIP, and on four video grounding datasets, V-HICO, DALY, YouCook-Interactions, and GroundingYouTube, showing that the proposed training-free approach is able to outperform current trained state-of-the-art approaches for spatial video grounding.

==> tables/verb_obj_act_weights.tex <==
\begin{center}
    \begin{table*}
        \begin{tabular}{ |p{2cm}|p{2.5cm}|p{5cm}||p{1cm}|p{1cm}|p{1cm}|p{1cm}|p{1cm}|  }
        
         \hline
         Prompt & Model &  Setting & VHICO & Daly & youCook & gr-YT & avg\\
         \hline
         
           && GEM baseline & 63.33 & 75.62 &  33.84 & 29.40 & 50.55\\
        & ViCLIP (vid) & GEM dynamic weights & 63.27 & 75.82&  34.00 & 29.62 & 50.68\\
           && GEM static weights & 64.66 & 76.20& 36.17 & 30.96 & 52.00\\
           && GEM static + dynamic weights & \textbf{64.72}  & \textbf{76.21} & \textbf{36.54}&  \textbf{31.26} & 52.18\\
         \cline{2-8}
        
           && GEM baseline & 64.17 & 75.87 & 32.64 & 28.40 & 50.27\\
         &ViCLIP (img) & GEM dynamic weights & 64.17 & 76.03 &32.60 &  28.62 & 50.36\\
           && GEM static weights & \textbf{65.44} & \textbf{76.35} & 34.16 & 29.67 & 51.41\\
           && GEM static + dynamic weights & 65.38 & 76.32 & \textbf{34.24} & \textbf{30.00} & 51.49\\
         \cline{2-8}
        
        
           && GEM baseline & 69.90 & 79.71 & 29.30 & 23.29 & 50.55\\
         &CLIP & GEM dynamic weights & 70.14 & 79.79 & 29.14 & 22.57 & 50.41 \\
           && GEM static weights & 72.32 & 82.06 &  \textbf{30.43} & \textbf{26.44} & 52.81\\
           && GEM static + dynamic weights & \textbf{72.80} & \textbf{82.48} & 29.74 & 25.69 & 52.68\\
         \cline{2-8}
        
           && GEM baseline & \textbf{70.87} & 78.65 & 41.16 & 17.75 & 52.11 \\
         Verb&OpenCLIP & GEM dynamic weights & 70.57 & 78.42 &  41.72 & 18.43 & 52.29\\
           && GEM static weights & 69.36 & \textbf{80.69} & 43.09 & 20.59 & 53.43\\
          & & GEM static + dynamic weights & 69.60 & 80.24 &  \textbf{43.45} & \textbf{21.60} & 53.72 \\
         \cline{2-8}
        
           && GEM baseline & 63.63& 64.75 & 33.00 & 31.18 & 48.17\\
         &BLIP & GEM dynamic weights & 64.66 & 65.45 & 33.20 & 31.41 & 48.68\\
           && GEM static weights & 68.15 & \textbf{68.23} &  44.86 & 40.41 & 55.41\\
           && GEM static + dynamic weights & \textbf{69.00} & 67.91 &  \textbf{45.54} &\textbf{40.49} & 55.74\\
         \cline{2-8}

         && GEM baseline & 66.38 & 74.92 & 33.99 & 26.00 & 50.33\\
        & AVG & GEM dynamic weights & 66.56 & 75.10 & 34.13 & 26.13 & 50.48\\
           && GEM static weights & 68.20 & 76.71 & 37.74 & 29.61 & 53.01\\
           && GEM static + dynamic weights & 68.3 & 76.63 & 37.90 & 29.81 & 53.16\\
         \hline




         && GEM baseline & \textbf{62.48} & 66.44 &  53.70 & 45.72 & 57.09\\
         &ViCLIP (vid) & GEM dynamic weights & 62.00 & 66.53 &  53.82 & 45.75 & 57.03\\
           && GEM static weights & 62.24 & \textbf{68.73} &  54.86 & 46.56 & 58.10\\
           && GEM static + dynamic weights & 62.30 & 68.71 & \textbf{54.94} & \textbf{46.78} & 58.18 \\
         \cline{2-8}
         
           && GEM baseline & 62.06 & 66.83 &  53.86 & 44.39 & 56.81\\
         &ViCLIP (img) & GEM dynamic weights & \textbf{62.18} & 66.92 & 53.98 & 44.63 & 56.93 \\
           && GEM static weights & 60.92 & 68.59 &  54.14 & 45.03 & 57.17 \\
           && GEM static + dynamic weights & 61.10 & \textbf{68.62} & \textbf{54.30} & \textbf{45.17} & 57.30\\
         \hline
        
           && GEM baseline & 65.74 & 76.27 &  46.50 & 36.24 & 56.19\\
         &CLIP (img) & GEM dynamic weights & \textbf{66.47} & 76.78 &  46.02 & 35.70 & 56.24\\
           && GEM static weights  & 65.68 & 78.70 &  \textbf{47.35} & \textbf{38.06} & 57.45\\
           && GEM static + dynamic weights & 65.56 & \textbf{79.45} & 47.19 & 37.52 & 57.43\\
         \cline{2-8}
        
           && GEM baseline & 67.55 & 76.43 & 49.68 & 28.35 & 55.50\\
        Object & OpenCLIP (img) & GEM dynamic weights & \textbf{68.52} & 75.67 & 50.76 & 30.91 & 56.47\\
           && GEM static weights & 64.90 & \textbf{77.86} & 50.96 & 32.03 & 56.44\\
          & & GEM static + dynamic weights & 65.44 & 77.00 & \textbf{51.21} &  \textbf{34.20} & 56.96\\
         \cline{2-8}
        
          & & GEM baseline & 59.95 & \textbf{59.85} & 32.68 & 34.17 & 46.66\\
         &BLIP (img) & GEM dynamic weights & 60.62 & 59.59 & 33.76 & 35.57 & 47.39\\
          & & GEM static weights & \textbf{62.48} & 58.09 & 45.34 & 40.27 & 51.55 \\
          & & GEM static + dynamic weights & 62.06 & 57.94 & \textbf{46.38} & \textbf{42.15} & 52.13\\
         \cline{2-8}

         && GEM baseline & 63.56 & 69.16 & 47.28 & 37.77 & 54.45\\
         &AVG & GEM dynamic weights & 63.96 & 69.10 & 47.67 & 38.51 & 54.81\\
          & & GEM static weights & 63.24 & 70.39 & 50.53 & 40.39 & 56.14 \\
          & & GEM static + dynamic weights & 63.29 & 70.34 & 50.80 & 41.16 & 56.4\\
         \hline

         
        
        \end{tabular}
        \caption{\textbf{Ablation for weights on verbs.} Accuracy for verb prompts with plain GEM (GEM baseline), GEM with dynamic weights added for the last three layers (GEM dynamic weights), GEM with static weights (GEM static weights), and a combination of static and dynamic weights (GEM static + dynamic weights).}
        \label{table:verb_weights}
        \vspace{-4mm}
    \end{table*}
\end{center}
